Continuous Monitoring of Pareto Frontiers on Partially Ordered Attributes for Many Users

We study the problem of continuous object dissemination---given a large number of users and continuously arriving new objects, deliver an object to all users who prefer the object. Many real world applications analyze users' preferences for effective object dissemination. For continuously arriving objects, timely finding users who prefer a new object is challenging. In this paper, we consider an append-only table of objects with multiple attributes and users' preferences on individual attributes are modeled as strict partial orders. An object is preferred by a user if it belongs to the Pareto frontier with respect to the user's partial orders. Users' preferences can be similar. Exploiting shared computation across similar preferences of different users, we design algorithms to find target users of a new object. In order to find users of similar preferences, we study the novel problem of clustering users' preferences that are represented as partial orders. We also present an approximate solution of the problem of finding target users which is more efficient than the exact one while ensuring sufficient accuracy. Furthermore, we extend the algorithms to operate under the semantics of sliding window. We present the results from comprehensive experiments for evaluating the efficiency and effectiveness of the proposed techniques.

==> sec-system_architecture.tex <==
\section{System Architecture}\label{sec:system_architecture}

Upon arrival of $o$, a naive approach computes for every user whether $o$ belongs to the Pareto-optimal objects. Consider an object $o'$ and a set of users $C' \subseteq C$ such that $o' \in \lambda_c(O)$ and $o \prec_c o'$ for each $c \in C'$. Because of this reason, for all $c \in C'$, the naive approach repeatedly compares $o$ with $o'$ total $n(C')$ times. Such repetitive comparisons increase time complexity. Our solution aims at countering this drawback. This section describes system architecture of our solution which comprises of three major components.

\subsection{Data Tables}
Fig.\ref{fig:structure} illustrates the components of our system architecture. We have two tables: dynamic Product Table and static User Table modeled by $O$ and $C$ (as given in Section~\ref{sec:model}), respectively. The  ever-growing Product Table allows insertion of a new object. It is very tiring to compute all target users upon the arrival of every new object in a large database. Our system architecture assists vendors to find target users in systematic and efficient way.

Table~\ref{tab:table_1} and Table~\ref{tab:table_2} correspond to data tables in the system architecture.

\subsection{Data Structure}

We have mentioned the drawback of naive approach at the beginning of this section. A case has been discussed considering two objects $o$, $o'$ and a set of users $C' \subseteq C$ where for every $c \in C'$, $o \prec_c o'$ and $o' \in \lambda_c(O)$. This implies that $(\forall c \in C': (\forall d \in \mathcal{D} : o.d=o'.d \vee o.d \prec_c^d o'.d) \wedge (\exists d \in \mathcal{D}  : o.d \prec_c^d o'.d))$. Consider a set of users $C'' \subseteq C'$ such that $\mathcal{D}$ can be partitioned into two disjoint sets $\mathcal{D} ^{=}$ and $\mathcal{D} ^{\prec}$ such that i) $\forall
d \in \mathcal{D} ^{=}$, $o.d$$=$$o'.d$ and ii) $\forall
d \in \mathcal{D} ^{\prec}$, $o.d$$\prec_c^d$$o'.d$. In other words, all users in $C''$ share common preference tuples tuples on values regarding $o$ and $o'$ with respect to all dimensions. Now, based on only one comparison between $o$ and $o'$, we can get that for all $c \in C''$, $o \prec_c o'$ , i.e., $o \notin \lambda_c(O)$.

\begin{example}
In Table~\ref{tab:table_1} and Table~\ref{tab:table_2}, if we compare $o_5$ with $o_2$ with respect to both $c_1$ and $c_2$, we get that $\mathcal{D} ^{\prec}$=\{\smallattrname{display size}, \smallattrname{brand}\} and $\mathcal{D} ^{=}$=\{\smallattrname{CPU cores}\}, since regarding both users, $o_4$ is dominated by $o_2$ on both \smallattrname{display size} and \smallattrname{brand} and both share same value on \smallattrname{CPU cores}. Hence, just based on single comparison, we can come decide that $o_4$ is not qualified for being Pareto-optimal with respect to any user.
\end{example}

It is intuitive from the aforementioned phenomenon that if $(\forall c \in C'' \forall o \in {O}^{\prec}: (\exists o' \in O-{O}^{\prec} : o \prec_c o'))$ then ${O}^{\prec} \not \subset \lambda_c(O)$. In other words, given a set of users having common preference tuples tuples on values with respect to all dimensions, comparisons with respect to partially ordered attributes representing common preference tuples tuples are enough in eliminating objects incapable of being Pareto-optimal with respect to each corresponding user. Considering ${O}^{\succeq}$ as Pareto-optimal object set with respect to that partially ordered attributes while ${O}^{\succeq} \subseteq O-{O}^{\prec}$, for all $c \in C''$ ${O}^{\succeq} \supseteq \lambda_c(O)$, i.e., ${O}^{\succeq}$ is enough in computing $\lambda_c(O)$.

In the data structure, we partition the set of all users $C$ into different disjoint sets $C_1$, $C_2$,...and $C_i$. In partitioning, we cluster all users based on \emph{similarity measurement of common preference tuples}. As standard clustering algorithms assume numeric data points, we redefine clustering algorithm for considering preferences on nominal values. Clustering is discussed further in Section~\ref{sec:system_architecture:clustering}.

Let $C_i$ comprises of users $c_{i1}$, $c_{i2}$,...and $c_{ij}$ while these users have common preference tuples tuples. Consider $c'_i$ as the shared common preference tuples tuples on values with respect to all dimensions of these users. We refer $c'_i$ and $c_{ij}$ as userHead and userMember of $C_i$, respectively.

We denote $C'$ as the set of all userHeads. Again $C^{c'}$ is the set of all userMembers in a certain cluster having userHead $c'$.

Consider $x$ and $y$ are two elements of $dom(d)$. Now $\forall d \in \mathcal{D} $, $(x,y) \in \prec_{c'}^d$ if and only if $(x,y) \in \prec_{c}^d$ for all $c \in C^{c'}$.

$\lambda_{c'_i}(O)$ denotes the set of Pareto-optimal objects with respect to $c'_i$. From aforementioned discussion, $\lambda_{c'_i}(O)$ is enough in computing $\lambda_{c_{i1}}(O)$, $\lambda_{c_{i2}}(O)$,...and $\lambda_{c_{ij}}(O)$. To represent $C_i$, the data structure contains $c'_i$ along with $c_{i1}$, $c_{i2}$,...and $c_{ij}$. It also maintains $\lambda_{c'_i}(O)$ along with $\lambda_{c_{i1}}(O)$, $\lambda_{c_{i2}}(O)$,...and $\lambda_{c_{ij}}(O)$ as well. We denote the storage of $\lambda_{c}(O)$ as $\mu_{c}$ regardless of whether $c$ denote userHead or userMember. In this paper, we use the terms $\lambda_{c}(O)$ (Pareto Frontier) and $\mu_{c}$ (storage of Pareto Frontier) alternatively.

So, the data structure consists of a number of different clusters. Each cluster has a userHead ($c'$) and corresponding userMembers ($C^{c'}$). For every cluster, $\mu_{c'}$ and $\mu_{c}$, i.e., $\forall c \in C^{c'}$ are maintained.

\begin{example}
In Table~\ref{tab:table_2}, we can think $c_1$ and $c_2$ form a cluster where $c'$ is created based on their common preference tupless. Consider $o_1$ to $o_{12}$ as existing tuples. We can see $\lambda_{c'}(O)$=$\{o_1, o_2, o_{10}, o_{12}\}$. To find out the Pareto-optimal objects with respect to $c_1$ and $c_2$, $\lambda_{c'}(O)$ is enough. Now the number of candidate Pareto-optimal objects is only 4 $(n(\lambda_{c'}(O)))$ instead of 12 $(n(O))$. We can see that $\lambda_{c_1}(O)$ contains only one Pareto-optimal object $o_1$. On the other hand, $o_1$, $o_2$ and $o_{12}$ belong to in $\lambda_{c_2}(O)$. In this case, the data structure contains $c'$, $c_1$ and $c_2$ along with corresponding Pareto Sets $\mu_{c'}$, $\mu_{c_1}$ and $\mu_{c_2}$, respectively. Storage of Pareto Sets are maintained upon insertion.\closedef
\end{example}

Upon the arrival of a new object, the data structure need to maintain its consistency. Let discuss what happens to $C_i$ for the arrival of new entry denoted as $o_{new}$. There can be three different cases.

Case I: If $o_{new}$ is dominated by any existing object $o$ in $\lambda_{c'_i}(O)$, then it is not Pareto-optimal with respect to $c'_i$. Hence, $o_{new}$ will remain non-Pareto optimal for all userMembers in ${C}_i$.

Case II: If $o_{new}$ dominates any existing object $o'$ in $\lambda_{c'_i}(O)$, then we need to update $\lambda_{c'_i}(O)$ as well as $\lambda_{C^{c'}}(O)$ for all $c \in C^{c'}$.  Now, $o_{new}$ belongs to $\lambda_{c'_i}(O)$. $o'$ is discarded from $\lambda_{c'_i}(O)$ as well as $\lambda_{C^{c'_i}}(O)$ for all $c \in C^{c'_i}$ such that $o' \in \lambda_{C^{c'_i}}(O-o_{new})$.

Case III: If $o_{new}$ is not dominated by any existing object in $\lambda_{c'_is}(O)$, then we need to update $\lambda_{c'_i}(O)$ as well as $\lambda_{C^{c'}}(O)$ for all $c \in C^{c'}$. After updating, $o_{new}$ is inserted to $\lambda_{c'_i}(O)$.

These cases are applicable for other clusters as well.

\begin{example}
Consider $o_{11}$ as a new tuple in Table~\ref{tab:table_1}.    As $o_{11}$ is not dominated by any object belongs to $\lambda_{c'}(O)$, $o_{11}$ is inserted into $\lambda_{c'}(O)$. Now regarding $c_1$, $o_{11}$ acts as a candidate for $\lambda_{c_1}(O)$. But $o_{11}$ is dominated by $o_2$ here. In case of $c_2$, $o_{11}$ dominates $o_5$ and $o_7$. Hence, both $o_5$ and $o_7$ are discarded from $\lambda_{c_2}(O)$ as well as $o_{11}$ takes place in $\lambda_{c_2}(O)$. Again, consider the insertion of $o_{12}$. As it is dominated by $o_2$, it is not Pareto-optimal with respect to $c'$. So, $o_{12}$ will remain non-Pareto optimal for all users in the corresponding cluster and thus no further computation is needed. Thus the data structure is maintained upon insertion.\closedef
\end{example}

\subsection{Clustering}\label{sec:system_architecture:clustering}
The intuition behind clustering is putting user having similar preferences together so that we can optimize computation through sharing computation across different dimensions. According to the description of our data structure, the benefit of optimization lies on the structure of userHead $c'$. Depending on $c'$, the set of candidate Pareto-optimal objects $\lambda_{c'}(O)$ is generated. We can assume $c'$ as a sieve through which $\lambda_{c'}(O)$ can pass and non-Pareto-optimal objects remain as residue.

Consider three users $c_1$, $c_2$, $c_3$ while in terms of similarity measurement $c_1$ is more similar to $c_2$ than $c_3$. Let the sets of non-Pareto-opbtimal objects with respect to $c_1$, $c_2$ and $c_3$ are $N_1$, $N_2$ and $N_3$. Considering a cluster of $c_1$ and $c_2$, let $c_{12}$ be the userHead and $N_{12}$ is corresponding set of non-Pareto-optimal objects. Similarly, considering a cluster of $c_1$ and $c_3$, let $c_{13}$ be the userHead and $N_{13}$ is corresponding set of non-Pareto-optimal objects. Here, $N_1 \cup N_2 \supseteq N_{12}$ and $N_1 \cup N_3 \supseteq N_{13}$. As $c_1$ is more similar to $c_2$, $(N_1 \cap N_2)-N_{12}$ is supposed to be smaller than $(N_1 \cap N_3)-N_{13}$. In other words, $c_{12}$ acts as better sieve than $c_{23}$ as we can get rid of more residue (non-Pareto-optimal objects with respect to each correspond user) for further computations. Intuitively, in a large dataset few objects qualify as being Pareto-optimal. Hence, most of the objects are non-Pareto optimal and discarding such objects just comparing respect to userHead is very cost pruning.

In this paper, we propose four different similarity functions for measuring similarity between two posets. We discuss these similarity functions considering two posets $\prec_{c_1}^d $ and $\prec_{c_2}^d $ while $d$ is a particular attribute.

\textbf{1) Intersection Similarity}\hspace{2mm} Intersection similarity is defined as the size of intersection, i.e., the number of common preference tuples.\\

$Intersection Similarity(d)$=$|\prec_{c_1}^d \cap \prec_{c_2}^d|$\\

\begin{example}
In Table~\ref{tab:table_2}, the common preference tuples between $c_1$ and $c_2$ on $CPU core$ are $( Dual$, $Single)$, $(Triple$, $Single)$ and $(Quad$, $Single)$. Hence, Intersection Similarity($CPU core$)=3.
\end{example}

\textbf{2) Jaccard Similarity}\hspace{2mm} Jaccard similarity is defined as the size of intersection divided by the size of the union of the preference tuples, i.e., the ratio of common preference tuples to all preference tuples.\\

$Jaccard Similarity(d)$=$\smash{|\prec_{c_1}^d \cap \prec_{c_2}^d| \over |\prec_{c_1}^d \cup \prec_{c_2}^d|}$\\

\begin{example}
In Table~\ref{tab:table_2}, on $CPU core$, $c_1$ and $c_2$ have 8 preference tuples in total including 3 common preference tuples. Hence, Jaccard Similarity($CPU core$)=3/8.
\end{example}

\textbf{3) Weighted Intersection Similarity}\hspace{2mm} Weighted Intersection Similarity is a modified version of Intersection Similarity. To discuss this, first we need to define \emph{suprema}.

\begin{definition}[Suprema]
With regard to $c$ and $d$, $x$ is a $supremum$ if it is not subsumed by any other value of $dom(d)$. The set of $d$'s suprema is denoted by $S_c^d$. In other words, it includes those attribute values over which no other value is preferred. Formally, $S_c^d$ = $\{x \in dom(d) | \nexists y \in dom(d) s.t. (y,x) \in \prec_{c}^d\}$.\closedef\vspace{-1.5mm}
\end{definition}

\begin{example}
In Table~\ref{tab:table_2}, with respect to $c_1$ and $CPU core$, $Dual$ is the only attribute value which is not subsumed by any other value, i.e., $S_{c_1}^{CPU core}$=$\{Dual\}$.
\end{example}

Regarding attribute $d$, consider $S_{c_1}^d$ and $S_{c_2}^d$ as the set suprema for user $c_1$ and $c_2$, respectively. In a particular poset, the weight of each node depends on its shortest distance from the suprema. Intuitively, as a node is closer to the suprema it is more preferable. Weighted Intersection Similarity is defined as the size of intersection along with the inverse distance from the suprema.\\

$Weighter Intersection Similarity(d)$=$${  {\displaystyle\sum_{(v, v') \in (\prec_{c_1}^d \cap \prec_{c_2}^d)} {\smash{1 \over \min_{\substack{
   si \in {S_{c_1}^d}
  }}
 dist(s_i,v)+1}\\\\+\smash{1 \over \min_{\substack{
   {s_i} \in {S_{c_2}^d}
  }}
 dist(s_i,v)+1}}} \over 2}$$\\

\begin{example}
In Table~\ref{tab:table_2}, on $CPU core$, $c_1$ and $c_2$ have common preference tuples $(Dual$, $Single)$, $(Triple$, $Single)$ and $(Quad$, $Single)$. As $Dual$ is a supremum for $c_1$, the minimum distance from suprema to $(Dual,Single)$ is 0.

$X(CPU core)$=[$1 \over {dist(Dual,Dual)+1}$+$1 \over {dist(Quad,Dual)+1}$\\\\+$1 \over {dist(Dual,Triple)+1}$+$1 \over {dist(Quad,Triple)+1}$\\\\+$1 \over {dist(Dual,Quad)+1}$+$1 \over {dist(Quad,Quad)+1}$]/2\\\\
=[$1$+$1 \over 3$+$1 \over 2$+$1 \over 2$+$1 \over 2$+$1$]/2\\\\
=1.92
\end{example}

\textbf{4) Weighted Jaccard Similarity}\hspace{2mm}\\ Weighted intersection is not enough as uncommon preference tupless are avoided here. It may be the case where there are large number of uncommon preference tupless. To tackle that issue we propose another similarity measure weighted Jaccard.

$Nominator(d)$=$Weighter Intersection Similarity(d)$\\
$Denominator(d)$=$Weighter Intersection Similarity(d)$\\\\$$+{\displaystyle\sum_{(v, v') \in (\prec_{c_1}^d-(\prec_{c_1}^d \cap \prec_{c_2}^d))} {\smash{1 \over \min_{\substack{
   s_i \in {S_{c_1}^d}
  }}
 dist(s_i,v)+1}}}$$\\\\$$+{\displaystyle\sum_{(v, v') (\prec_{c_2}^d-(\prec_{c_1}^d \cap \prec_{c_2}^d))} {\smash{1 \over \min_{\substack{
   s_i \in {S_{c_2}^d}
  }}
 dist(s_i,v)+1}}}$$\\

\begin{example}
In Table~\ref{tab:table_2}, other than common ones, $c_1$, $c_2$ have these preference relations $\{(Dual,Triple)$, $(Dual,Quad)\}$ and $\{(Quad,Triple)$, $(Quad,Dual)$, $(Triple,Dual)\}$, respectively.

Denominator($CPU core$)=1.92+$1 \over {dist(Dual,Dual)+1}$+\\\\$1 \over {dist(Dual,Dual)+1}$+$1 \over {dist(Quad,Quad)+1}$\\\\+$1 \over {dist(Quad,Quad)+1}$+$1 \over {dist(Quad,Triple)+1}$\\\\
=6.42
\end{example}

Let denote similarity measurement on $d$ as $SM(d)$ in general. As different dimension can have different number of attribute values, the similarity measurement with respect to all attributes $SM$ is computed after normalizing $SM(d)$.\\

$SM$=$\sum_{{SM(d_i) \over |dom(d_i)|}}$

%Here is more analysis. Consider a cluster of $n$ different users. In the worst case, $c'$ is $\phi$ (no common preference tuples relation). In this case, no object is not going to be pruned by $c'$, i.e, $\lambda_{c'}(O)$=$O$. In the best scenario, all users have identical preference orders. Now $c'$ is same as each user profile. And $\delta{c_1}$=$\delta{c_2}$=...=$\delta{c_n}$=$\phi$. Here all the computations are done in $c'$. In terms of time complexity, it is $n$ times faster than baseline.%

\subsection{Query Processing}

Consider $o_q$ as an element of $O$. We want to know the target users $C^{o_q}$, i.e., $\{c| c \in C, o_q \in \lambda_{c}(O)\}$. For this, regarding each cluster we need to do the same operation. Let consider $C_1$.

Case I: If $o_q$ belongs to $O-\lambda_{c'_1}(O)$, then this cluster doesn't contain any element of $C^{o_q}$.

Case II: If If $o_q$ belongs to $\lambda_{c'_1}(O)$, then this cluster may contain elements of $C^{o_q}$. We need to look through all Pareto-optimal objects of each corresponding user. If any user contain $o_q$ as one of its Pareto-optimal objects, then it will be an element of $C^{o_q}$. As for each user the data structure is storing Pareto-optimal objects only, $C^{o_q}$ does not include any user other than target users.

\begin{example}
In Table~\ref{tab:table_2}, suppose we are looking for the target users of $o_1$ of Table~\ref{tab:table_1},. As $o_1$ does not belong to $O'$, the there is no target user of $o_1$. Consider $o_2$ as $o_q$. As $o_2$ belongs to $O'$, we need to look through all users of the corresponding cluster. The target users of $o_2$ are both $c_1$ and $c_2$.\closedef
\end{example}

\begin{figure}[t]
\centering
\epsfig{file=images/structure.eps,scale=0.5}\vspace{-2mm}
\caption{System Architecture}\vspace{-4mm}
\label{fig:structure}
\end{figure}

